OpenForge: Probabilistic Metadata Integration

Modern data stores increasingly rely on metadata for enabling diverse activities such as data cataloging and search. However, metadata curation remains a labor-intensive task, and the broader challenge of metadata maintenance -- ensuring its consistency, usefulness, and freshness -- has been largely overlooked. In this work, we tackle the problem of resolving relationships among metadata concepts from disparate sources. These relationships are critical for creating clean, consistent, and up-to-date metadata repositories, and a central challenge for metadata integration. We propose OpenForge, a two-stage prior-posterior framework for metadata integration. In the first stage, OpenForge exploits multiple methods including fine-tuned large language models to obtain prior beliefs about concept relationships. In the second stage, OpenForge refines these predictions by leveraging Markov Random Field, a probabilistic graphical model. We formalize metadata integration as an optimization problem, where the objective is to identify the relationship assignments that maximize the joint probability of assignments. The MRF formulation allows OpenForge to capture prior beliefs while encoding critical relationship properties, such as transitivity, in probabilistic inference. Experiments on real-world datasets demonstrate the effectiveness and efficiency of OpenForge. On a use case of matching two metadata vocabularies, OpenForge outperforms GPT-4, the second-best method, by 25 F1-score points.

==> sections/06_discussion.tex <==
\section{Discussion}\label{sec:discussion}

% \subsection{Sequential Modeling}
%   Recall that each message passing in MRF inference has $O(nk^{2})$ time and space complexity where $n$ is the number of random variables in MRF and $k$ is the number of states of each random variable. With more relation types (i.e., more states of each random variable), the inference cost will increase quadratically in time and space. The dependency among random variables (imposed by the relation transitivity) will also become more complex. Additionally, more number of relation types to resolve in one joint space will require more diverse features to learn effective ML priors that can distinguish between different relation types. These factors can pose significant challenges for MRF modeling and any other solution.

%   Having more RAM and GPU memory will help scale our MRF modeling approach as analyzed in the scalability experiments. Nevertheless, to extend our approach for resolving more relation types in practice or working with constrained resources such as RAM, we recommend a scheme of sequential modeling. The idea is to resolve one type of relation in each run and reduce the time and space complexity by using a MRF consisting of binary random variables. For instance, we can use our MRF modeling apporach to resolve the equivalence relation in the first run and then plug in the predictions as evidence to resolve another relation type in the next run and so on. In this way, we can resolve multiple relation types in a sequential manner, thereby managing algorithmic complexity and avoiding memory blow up.  

\subsection{The State of Metadata}
 Metadata associated with datasets (e.g., in governmental Open Data portals) can be incomplete or inconsistent, and may exhibit various levels of semantic granularity~\cite{DBLP:journals/debu/MillerNZCPA18}. For this reason, many works involving Open Data do not consider metadata in their solutions~\cite{DBLP:journals/pvldb/ZhuNPM16, DBLP:journals/pvldb/NargesianZPM18, DBLP:journals/pvldb/NargesianZMPA19, DBLP:journals/pacmmod/KhatiwadaFSCGMR23, DBLP:journals/corr/CongNJ23}. While we agree this criticism is valid in some circumstances, we draw attention to the other side of the state of metadata. That is, there is an increasing existence of metadata in many online data repositories~\cite{ICPSR, HarvardDataverse, DataGov, NYCOpenData, GOODS} and existing metadata can already provide useful contextual information as shown in~\cite{XingARTS23} and this work. Examples of high-quality metadata include dataset and column descriptions existent for many datasets archived by governmental Open Data portals~\cite{DataGov, NYCOpenData}, social and behavioral science data platforms~\cite{ICPSR,HarvardDataverse} and Google~\cite{GOODS, DBLP:conf/sigmod/HalevyKNOPRW16}. 

  It is worth mentioning that regardless of availability of metadata for Open Data repositories, the usability of datasets in the repositories, especially for domain experts, such as journalists, social scientists, and publicy makers, crucially depends on the existence of metadata~\cite{alter2012response, ember2013sustaining}. This emphasizes the need for inferring and standardizing metadata for and across these repositories.

  % \fn{Need to mentions and cite more approaches from the NLP side for extracting hypernym relations or refer to the related work section.} 
  % Researchers in natural language processing community have been using Hearst patterns~\cite{DBLP:conf/coling/Hearst92} to automatically extract hypernym relation from text corpora~\cite{DBLP:conf/coling/Hearst92, DBLP:conf/nips/SnowJN04, DBLP:conf/acl/SnowJN06, DBLP:conf/emnlp/RollerE16, DBLP:conf/acl/RollerKN18}. Similarly, we hypothesize and show that it is possible to extract and induce a taxonomy of concepts from free-text metadata of a dataset corpus, which can be used to consistently describe data in the corpus. In particular, we standardize the extracted noisy vocabulary and infer a taxonmy on this vocabulary by resolving various relations between concepts.
